IP Neo-colonialism: Geo-auditing RIR Address Registrations

Allocation of the global IP address space is under the purview of IANA, who distributes management responsibility among five geographically distinct Regional Internet Registries (RIRs). Each RIR is empowered to bridge technical (e.g., address uniqueness and aggregatability) and policy (e.g., contact information and IP scarcity) requirements unique to their region. While different RIRs have different policies for out-of-region address use, little prior systematic analysis has studied where addresses are used post-allocation. In this preliminary work, we e IPv4 prefix registrations across the five RIRs (50k total prefixes) and utilize the Atlas distributed active measurement infrastructure to geolocate prefixes at RIR-region granularity. We define a taxonomy of registration ``geo-consistency'' by comparing a prefixes' inferred physical location to the allocating RIR's coverage region as well as the registered organization's location. We then apply this methodology and taxonomy to audit the geo-consistency of 10k random IPv4 prefix allocations within each RIR (50k total prefixes). While we find registry information to largely be consistent with our geolocation inferences, we show that some RIRs have a non-trivial fraction of prefixes that are used both outside of the RIR's region and outside of the registered organization's region. A better understanding of such discrepancies can increase transparency for the community and inform ongoing discussions over in-region address use and policy.

==> ethics.tex <==
\section{Ethics}

We abide by the RIR's Acceptable Use Policies.  This work does not raise any ethical issues.

